Heuristic Rectangle Splitting: Leveraging Single-Objective Heuristics to Efficiently Solve Multi-Objective Problems

Real-life problems are often characterized by conflicting optimization objectives. Consequently, there has been a growing interest not only in multi-objective models, but also in specialized multi-objective metaheuristics for solving those models. A wide variety of methods, e.g. NSGA-II, SPEA, IBEA, scatter search, Pareto local search, and many others, have thus been proposed over the years. Yet in principle, multi-objective problems can be efficiently solved with existing tailored single-objective solvers -- this is the central idea behind the well-known epsilon-constraint method (ECM). Despite its theoretical properties and conceptual simplicity, the epsilon-constraint method has been largely ignored in the domain of heuristics and remains associated mostly with exact algorithms. In this article we dispel these preconceptions and demonstrate that the epsilon-constraint framework can be a highly effective way to directly leverage the existing research on single-objective optimization for solving multi-objective problems. We propose an improved version of the classical ECM adapted to the challenges and requirements specific to heuristic search. The resulting framework is implemented with an existing state-of-the-art single-objective solver for the Capacitated Vehicle Routing Problem (CVRP) and tested on the VRP with Route Balancing (VRPRB). Based on an extensive computational study, we show the added value of our adaptations compared to the classical ECM, and demonstrate that our simple epsilon-constraint algorithm significantly outperforms the current state-of-the-art multi-objective metaheuristics with respect to multiple quality metrics. We conclude with a discussion of relevant success factors and promising directions for further research.

==> sections/4-conventions.tex <==
\section{Computational Setting}
\label{4-conventions}

This section briefly explains the performance indicators and states the parameter settings used in our computational study.

%\input{sections/4-1-conventions}
\input{sections/4-2-indicators}
\input{sections/4-3-parameters}


